Visual Reinforcement Learning with Imagined Goals

For an autonomous agent to fulfill a wide range of user-specified goals at test time, it must be able to learn broadly applicable and general-purpose skill repertoires. Furthermore, to provide the requisite level of generality, these skills must handle raw sensory input such as images. In this paper, we propose an algorithm that acquires such general-purpose skills by combining unsupervised representation learning and reinforcement learning of goal-conditioned policies. Since the particular goals that might be required at test-time are not known in advance, the agent performs a self-supervised "practice" phase where it imagines goals and attempts to achieve them. We learn a visual representation with three distinct purposes: sampling goals for self-supervised practice, providing a structured transformation of raw sensory inputs, and computing a reward signal for goal reaching. We also propose a retroactive goal relabeling scheme to further improve the sample-efficiency of our method. Our off-policy algorithm is efficient enough to learn policies that operate on raw image observations and goals for a real-world robotic system, and substantially outperforms prior techniques.

==> em.tex <==

We formalize the problem with the graphical mode shown in Figure \ref{fig:pgm-v1}.
\begin{figure}
    \centering
    \begin{tikzpicture}
       \node[state] (s0) at (0,0) {$s_0$};
       \node[state] (z0) at (0,1.5) {$z_0$};
       \node[state] (o0) at (0,3) {$o_0$};
       \node[state, fill=gray!25] (w0) at (0,4.5) {$\Omega_0$};
       \node[state] (a0) at (1.5,1.5) {$a_0$};

       \node[state] (s1) at (3,0) {$s_1$};
       \node[state] (z1) at (3,1.5) {$z_1$};
       \node[state] (o1) at (3,3) {$o_1$};
       \node[state, fill=gray!25] (w1) at (3,4.5) {$\Omega_1$};
       \node[state] (a1) at (4.5,1.5) {$a_1$};
       
       \node[state] (s2) at (6,0) {$\cdots$};
       
       \node[state] (z0g) at (0,7.5) {$z_0^g$};
       \node[state] (o0g) at (0,6) {$o_0^g$};
       
       \node[state] (z1g) at (3,7.5) {$z_1^g$};
       \node[state] (o1g) at (3,6) {$o_1^g$};

       \draw[every loop]
            (s0) edge node {} (z0)
            (s0) edge node {} (s1)
            (z0) edge node {} (o0)
            (o0) edge node {} (a0)
            (o0) edge node {} (w0)
            (a0) edge node {} (s1)
            
            (s1) edge node {} (z1)
            (s1) edge node {} (s2)
            (z1) edge node {} (o1)
            (o1) edge node {} (a1)
            (o1) edge node {} (w1)
            (a1) edge node {} (s2)
            
            (z0g) edge[bend left] node {} (a0)
            (z1g) edge[bend left] node {} (a1)

            (z0g) edge node {} (o0g)
            (o0g) edge node {} (w0)
            
            (z1g) edge node {} (o1g)
            (o1g) edge node {} (w1)
            ;
    \end{tikzpicture}
    \caption{Version 1 graphical model for self-supervised learning}
    \label{fig:pgm-v1}
\end{figure}

The parts of the graph are
\begin{itemize}
    \item $Z_t^g$ is a goal latent
    \item $O_t^g$ is a goal observation
    \item $\Omega_t^g$ is an optimality variable which equals $1$ if $O_t^g$ and $O_t$ are the same
    \item $S_t$ is a true underlying state
    \item $A_t$ is the action taken, whose distribution is the policy $\pi_\theta(\cdot \mid o_o, z_o^g)$.
    \item $Z_t$ is a reached latent
    \item $O_t$ is a reached observation
\end{itemize}
We assume that all the probability distributions are fixed (and unknown) except for $p_\theta(a_t \mid o_t, z^g_o)$ which we parameterize by $\theta$.
We'll write $p_\theta(X=x)$ to mean the PDF of the random variable $X$ evaluated at the value $x$.
We'll leave $\theta$ in the subscript to remind ourselves if the PDF (or expectation) depends on $\theta$.
This might seem verbose, so we'll only use it when writing tricky equations like $\E_\theta[ p_\theta(O_t= O_t^g)]$ to remember that this should be read as
\[
\int_{\mathcal O_t} p_\theta(O_t = x) p_\theta(O_t^g = x) dx.
\]
If the meaning is obvious, we'll just write $p(x)$ to mean $p_\theta(X=x)$.

We formalize the problem as
\begin{align}
\max_\theta \log \E_\theta [ p_\theta(\Omega_{1:T}=1)] . 
\end{align}
Remember that $\Omega_t$ is the event that $O_t^g$ and $O_t$ are the same.
So, using this fact and Jensen's inequality, we can rewrite this as
\begin{align}
\max_\theta \log \E_\theta [ p_\theta(\Omega{1:T}=1)]
&= \max_\theta \log \E_\theta [ \E_\theta [ p_\theta(\Omega_{1:T}=1) ] \mid O_{1:T}^g]
\\&=\max_\theta \log \E_\theta [ \E_\theta [ p_\theta(O_{1:T} = O_{1:T}^g)] \mid O_{1:T}^g]
\\&\geq\max_\theta \E_\theta [ \E_\theta [ \log p_\theta(O_{1:T} = O_{1:T}^g)] \mid O_{1:T}^g]
\\&\triangleq \max_\theta \mathcal{F}(\theta)
\end{align}
Our method can be seen as performing EM \textbf{on this lower bound}, where the latents to marginalize out are the latents $z$.
Note that EM has its own lower bound and should be not confused with the fact that $\mathcal F$ is a lower bound for our true objective.
EM works by lower-bounding the inner $\log p_\theta(O_{1:T} = o_{1:T}^g)$ term.
Here, we use a lower-case $o_{1:T}^g$ to remind ourselves that the goal observations should not be considered random variables inside the expectation.
\begin{align}
\log p_\theta(O_{1:T} = o_{1:T}^g)]
&= \log \E_{\zeta_{1:T} \sim q}[
    \frac{
        p_\theta(O_{1:T} = o_{1:T}^g, Z_{1:T}=\zeta_{1:T})
    }{
        q(Z_{1:T} = \zeta_{1:T} \mid O_{1:T} = o_{1:T}^g)
    }
]
\\
&\geq \E_{\zeta_{1:T} \sim q}[ \log
    \frac{
        p_\theta(O_{1:T} = o_{1:T}^g, Z_{1:T}=\zeta_{1:T})
    }{
        q(Z_{1:T} = \zeta_{1:T} \mid O_{1:T} = o_{1:T}^g)
    }
]
\\
&\triangleq \mathcal L(q, \theta)
\end{align}
EM optimizes $\mathcal L(q, \theta)$ by alternating between optimizing the model parameters $\theta$ and the variational distribution $q$.
In the ``E'' step does
\[
    q = \text{argmax}_q \mathcal L(q, \bar \theta)
\]
and the ``M'' step does
\[
    \theta = \text{argmax}_\theta \mathcal L(\bar q, \theta)
\]
with the bar indicating that the variable is treated as a constant.
\subsection{E step}
% The class of variational distributions is very important, with two natural candidates are
% \begin{align}
%     q(Z_{1:T} \mid O_{1:T}) = \begin{cases}
%         \prod_t q(Z_t \mid O_t) & \text{VAE}\\
%         \prod_t q(Z_t \mid O_{1:t}) & \text{RNN+VAE}
%     \end{cases}
% \end{align}
The E step can be written as
% \begin{align}\label{eq:lb-vae-term}
% \mathcal L(q, \theta)
% &= \E_{\zeta_{1:T} \sim q}[ \log
%     p_\theta(O_{1:T} = o_{1:T}^g \mid Z_{1:T}=\zeta_{1:T})
% ]
% \\\nonumber
% &\qquad
% + KL(
%     q(Z_{1:T} = \cdot \mid O_{1:T} = o_{1:T}^g)
% ||
%     p_\theta(Z_{1:T}=\cdot)
% )
% \end{align}
% or simply
\begin{align}\label{eq:lb-vae-term}
\max_q \mathcal L(q, \theta)
&=
\max_q
\E_q[ \log
    p_\theta(o_{1:T}^g \mid \zeta_{1:T})
]
+ KL(
    q( \cdot \mid o_{1:T}^g)
||
    p_\theta(\cdot)
) 
\end{align}
If we both $p_\theta$ and $q$ to factorize over time, we get
\begin{align}
\max_q \mathcal L(q, \theta)
&=
\max_q
\sum_t \E_q[ \log
    p_\theta(o_t^g \mid \zeta_t)
]
+ KL(
    q( \cdot \mid o_t^g)
||
    p_\theta(\cdot)
) 
\end{align}
which is exactly the VAE loss.
Note that just as in VAEs, we do not actually know $p_\theta$ and so we model it using a decoder that we train with MLE.

==> pgm.tex <==
\begin{figure}
    \centering
    \begin{tikzpicture}
       \node[state] (s0) at (0,0) {$s_0$};
       \node[state] (z0) at (0,1.5) {$z_0$};
       \node[state, fill=gray!25] (o0) at (0,3) {$o_0$};
       \node[state, fill=gray!25] (w0) at (0,4.5) {$\Omega_0$};
       \node[state] (u0) at (1.5,1.5) {$u_0$};

       \node[state] (s1) at (3,0) {$s_1$};
       \node[state] (z1) at (3,1.5) {$z_1$};
       \node[state, fill=gray!25] (o1) at (3,3) {$o_1$};
       \node[state, fill=gray!25] (w1) at (3,4.5) {$\Omega_1$};
       \node[state] (u1) at (4.5,1.5) {$u_1$};

       \node[state] (sg) at (11.5,4.5) {$s_g$};
       \node[state] (zg) at (10,4.5) {$z_g$};
       \node[state, fill=gray!25] (og) at (10,3) {$o_g$};

       \draw[every loop]
            (s0) edge node {} (z0)
            (z0) edge node {} (o0)
            (o0) edge node {} (u0)
            (z0) edge[bend left] node {} (w0)
            (u0) edge node {} (s1)
            (s1) edge node {} (z1)
            (z1) edge node {} (o1)
            (o1) edge node {} (u1)
            (z1) edge[bend left] node {} (w1)

            (sg) edge node {} (zg)
            (zg) edge node {} (og)

            % (u1) edge node {} (s1)
            (zg) edge[bend right] node {} (w0)
            (zg) edge[bend right] node {} (w1);
    \end{tikzpicture}
    \caption{A graphical model for self-supervised learning}
    \label{fig:pgm}
\end{figure}
